Large Deviations for Accelerating Neural Networks Training

Artificial neural networks (ANNs) require tremendous amount of data to train on. However, in classification models, most data features are often similar which can lead to increase in training time without significant improvement in the performance. Thus, we hypothesize that there could be a more efficient way to train an ANN using a better representative sample. For this, we propose the LAD Improved Iterative Training (LIIT), a novel training approach for ANN using large deviations principle to generate and iteratively update training samples in a fast and efficient setting. This is exploratory work with extensive opportunities for future work. The thesis presents this ongoing research work with the following contributions from this study: (1) We propose a novel ANN training method, LIIT, based on the large deviations theory where additional dimensionality reduction is not needed to study high dimensional data. (2) The LIIT approach uses a Modified Training Sample (MTS) that is generated and iteratively updated using a LAD anomaly score based sampling strategy. (3) The MTS sample is designed to be well representative of the training data by including most anomalous of the observations in each class. This ensures distinct patterns and features are learnt with smaller samples. (4) We study the classification performance of the LIIT trained ANNs with traditional batch trained counterparts.

==> LADNN/Other/methodology_old.tex <==
# Our LDP Model
We plan to use LDP to identify the presence of large deviations (or anomalous) observations. We use the shift in the observed mean as a means to study outlier observations. Let $a_n$ be an external observation added to $\{X_i\}_{i=1}^N$ cluster of size N (mean $=0$, variance 1 say). Two time steps exists:




<!-- Before adding $a_n$ :

$\mu_n = \frac{\sum X_i}{N}$
 -->
<!-- After adding $a_n$:

$\mu_{n+1}= \epsilon = \frac{a_n+\sum X_i}{N+1}$
 -->

By LDP, $P(\frac{\sum_{i=1}^{N+1} X_i}{N+1} \geq \epsilon)=e^{-\epsilon^2*(N+1)/2}
$

If expected mean$=\hat{\mu}$ and variance$=\hat{\sigma}^2/N$, then by standardizing, we get,

$P(\frac{\frac{\sum_{i=1}^{N+1} X_i}{N+1}-\mu}{(\sigma/\sqrt{N})}  \geq \epsilon)=e^{-\epsilon^2*(N+1)/2}
$ where, $\mu=\mu_n =\frac{\sum x_i}{N}$ was mean before adding $a_n$.

$P(\frac{\frac{\sum_{i=1}^{N+1} X_i}{N+1}-\mu}{(\sigma/\sqrt{N})}  \geq \epsilon)=e^{-\epsilon^2*(N+1)/2}
$ and $\epsilon = \frac{\frac{a_n+\sum x_i}{N+1}-\mu}{(\sigma/\sqrt{N})} $ and let $\sum x_i=x_.$(Say). Then, 

$ \epsilon = \frac{\frac{a_n+x_.}{N+1}-\frac{x_.}{N}}{(\sigma/\sqrt{N})} $
$= \frac{\frac{N*a_n+N*x_.-(N+1)*x_.}{N*(N+1)}}{(\sigma/\sqrt{N})} $

$= \frac{N*a_n-x_.}{N*(N+1)(\sigma/\sqrt{N})} $

$= \frac{a_n-\mu}{(N+1)(\sigma/\sqrt{N})} $



NOTE: In the inequality, LHS is the r.v. and RHS is its realization.




<!-- $P(\mu_n\geq \epsilon)=e^{-\epsilon^2/2}
$


$P(shift\_in\_mean \geq \epsilon)=P(|\mu_n-\mu_{n+1}|\geq \epsilon)$

$=P(\mu_n - \mu_{n+1}\geq \epsilon)$ (without loss of generality say new mean is less than old mean)

$=P(\mu_n \geq \mu_{n+1} + \epsilon)$ 

$=e^{-\{\mu_{n+1} + \epsilon\}^2/2}
$

(if new mean is greater than old mean)

$P(shift\_in\_mean \geq \epsilon)=P(|\mu_n-\mu_{n+1}|\geq \epsilon)$

$=P(\mu_{n+1}- \mu_n \geq \epsilon)$ 

$=P(- \mu_n \geq -\mu_{n+1}+ \epsilon)$ 

$=P(\mu_n \leq \mu_{n+1}-\epsilon)$ 

$=1- P(\mu_n \geq \mu_{n+1}-\epsilon)$ 

$=1- e^{-\{\mu_{n+1} - \epsilon\}^2/2}$ 

 -->

==> LADNN/Other/points.tex <==
% Paper Makeup: Page Limit 9
% Abstract        - 0.25
% Introduction    - 1
% Lit. Review     - 1
% Background      - 1
% Methodology     - 2
% Results         - 3
% Conclusion      - 0.5
% References      - 1

\section{Paper flow and points to be included}
\begin{enumerate}
    \item Abstract, Intro and contributions in brief:
    \begin{enumerate}
        \item Anomaly detection only using LDP
        \item AD and clustering using LDP with clustering algorithm
        \item AD and clustering using LDP only
        \item LDP on COVID19 data
    \end{enumerate}
    \item Lit Review:
    \begin{enumerate}
        \item LDP used in AD
        \item LDP use in clustering
        \item Why EVT is lacking? Why do we need new model?
        \item Why combine with clustering methods?
    \end{enumerate}
    \item Methodology:
    \begin{enumerate}
        \item LDP Background and theorems
        \item LDP for dimensionality reduction in AD
        \item LDP for clustering
        \item Algorithms for each of the models
    \end{enumerate}
    \item Model Contributions:
    \begin{enumerate}
        \item LDP on COVID
        \item LDP for dimensionality reduction in AD
        \item LDP based clustering
    \end{enumerate}
    \item Results:
    \begin{enumerate}
        \item ODDS data
        \item COVID Data
        \item Clustering data
        \item How LDP is better than EVT for high dimensions
        \item Is LDP faster than EVT, CRP or INCAD?
        \item Is performance improving?
        \item Is separability is preserved in dimensionality reduction?
        \item Stream data?? TRY LATER
    \end{enumerate}
\end{enumerate}

==> LADNN/abstract.tex <==
\begin{abstract}

\end{abstract}



==> LADNN/ldp_background.tex <==
\section{Large Deviation Principle}\label{ldp_background}
Large deviations theory provides techniques to derive the probability of rare events\footnote{In our context, these rare events include outlier/anomalous behaviors.} %The theory provides a powerful way of handling the anomaly probabilities of rare events 
that have an asymptotically exact exponential approximation\cite{den2008large, varadhan1984large, varadhan2010large}. 
%
In this section, we briefly go over the large deviation theory and different ways to generate the rate functions required for the large deviations principle.

The key concept of this theory is the Large Deviations Principle (LDP). The principle describes the exponential decay of the probabilities for the mean of random variables. The rate of decay is characterized by the rate function $\mathcal{I}$. The theorem is detailed below:

\begin{theorem}\label{ldp_theorem}
    A family of probability measures $\{\mu_\epsilon\}_{\epsilon>0}$ on a Polish space $\mathcal{X}$ is said to satisfy large deviation principle (LDP) with the rate function $\mathcal{I}:\mathcal{X}\to[0,\infty]$ if:
    \begin{enumerate}
        \item $\mathcal{I}$ has compact level sets and is not identically infinite
        \item $lim inf_{\epsilon \to 0} \epsilon log\mu_\epsilon(\mathcal{O})\geq-\mathcal{I}(\mathcal{O}) \quad \forall \mathcal{O}\subseteq \mathcal{X}$ open sets
        \item $lim sup_{\epsilon\to0} \epsilon log\mu_\epsilon(\mathcal{C}) \leq-\mathcal{I}(\mathcal{C}) \quad \forall \mathcal{C}\subseteq \mathcal{X}$ closed sets
    \end{enumerate}
where, $\mathcal{I}(\mathcal{S})=inf_{x\in \mathcal{S}}\mathcal{I}(x),\ \mathcal{S}\subseteq\mathcal{X}$ 
\end{theorem}

% \begin{theorem}\label{ldp_theorem}
%     A family of probability measures $\{\mu_\epsilon\}_{\epsilon>0}$ on a Polish space $\mathcal{X}$ is said to satisfy large deviation principle (LDP) with the rate function $\mathcal{I}:\mathcal{X}\to[0,\infty]$ if:
%     \begin{enumerate}
%         \item $\mathcal{I}$ has compact level sets and is not identically infinite
%         \item \begin{equation}
%                 \begin{aligned}
%                     lim inf_{\epsilon \to 0} \epsilon &log\mu_\epsilon(\mathcal{O}) \geq-\mathcal{I}(\mathcal{O}), \\
%                     & \forall \mathcal{O}\subseteq \mathcal{X} 
%                     \text{ open sets}
%                 \end{aligned}
%             \end{equation}
%     \item \begin{equation}
%                 \begin{aligned}
%                 lim sup_{\epsilon\to0} \epsilon &log\mu_\epsilon(\mathcal{C}) \leq-\mathcal{I}(\mathcal{C}), \\ 
%                 &\forall \mathcal{C}\subseteq \mathcal{X}                     \text{ closed sets}                
%                 \end{aligned}
%             \end{equation}
%     \end{enumerate}
% where, $\mathcal{I}(\mathcal{S})=inf_{x\in \mathcal{S}}\mathcal{I}(x),\ \mathcal{S}\subseteq\mathcal{X}$ 
% \end{theorem}

% Some of the properties of the rate function are given by Varadhan's Lemma and Bryc's Lemma. 
% \begin{theorem}{Varadhan's Lemma }
%     If $\{\mu_\epsilon\}_{\epsilon>0}$ satisfies the LDP on $\mathcal{X}$ with rate function $\mathcal{I}$ then, 
% \begin{equation}
% \begin{aligned}
%     lim_{\epsilon\to 0} \epsilon log \int_{\mathcal{I}}e^{F(x)/\epsilon}\mu_\epsilon(dx)=\Lambda_F\quad \forall F\in \mathrm{C}_b(\mathcal{X})
% \end{aligned}    
% \end{equation}
% where $\mathrm{C}_b(\mathcal{X})$ is the space of continuous bounded functions on $\mathcal{X}$ and

% \begin{equation}
%     \begin{aligned}
%     \Lambda_F=sup_{x\in\mathcal{X}}\left[ F(x)-\mathcal{I}(x)\right]
%     \end{aligned}
% \end{equation}
% \end{theorem}

% \begin{theorem}{Bryc's Lemma}
% Suppose $\{\mu_\epsilon\}_{\epsilon>0}$ is exponentially tight and the limit in Varadhan's lemma exits $\forall F\in \mathrm{C}_b(\mathcal{X})$. Then, $\{\mu_\epsilon\}_{\epsilon>0}$ satisfies LDP with rate function $\mathcal{I}$ given by
% \begin{equation}
%     \begin{aligned}
%     \mathcal{I}(x)=sup_{F\in \mathrm{C}_b(\mathcal{X})}\left[F(x)-\Lambda_F \right]\quad x\in\mathcal{X}
%     \end{aligned}
% \end{equation}
% \end{theorem}

To implement LDP on known data with known distributions, it is important to decipher the rate function $\mathcal{I}$. Cramer's Theorem provides the relation between the rate function $\mathcal{I}$ and the logarithmic moment generating function $\Lambda$. 
% These results are useful to determine $\mathcal{I}$ for random varibales of 

\begin{definition}
The logarithmic moment generating function of a random variable $X$ is defined as
\begin{equation}
    \begin{aligned}
        \Lambda(t)=\log E[\exp(tX)]
    \end{aligned}
\end{equation}
\end{definition}

\begin{theorem}[Cramer's Theorem]
Let $ X_1, X_2, \dots X_n$ be a sequence of iid real random variables with finite logarithmic moment generating function, e.g. $\Lambda(t)<\infty$ for all $t\in\mathbb{R}$.
Then the law for the empirical average satisfies the large deviations principle with rate $\epsilon=1/n$ and rate function given by
\begin{equation}
    \begin{aligned}
        \mathcal{I}(x):= \sup_{t \in \mathbb{R}} \left(tx-\Lambda(t) \right) \quad \forall t\in\mathbb{R}
    \end{aligned}
\end{equation}
% Then the Legendre transformation of $\Lambda$ given by $$\Lambda^*(x):= \sup_{t \in \mathbb{R}} \left(tx-\Lambda(t) \right)$$
% satisfies, 
% $$\lim_{n \to \infty} \frac{1}{n} \log \left(P\left(\sum_{i=1}^n X_i \geq nx \right)\right) = -\Lambda^*(x),\quad \forall x > E[X_1]$$.
\end{theorem}
Thus, we get, 
\begin{equation}
    \begin{aligned}
    \lim_{n \to \infty} \frac{1}{n} \log \left(P\left(\sum_{i=1}^n X_i \geq nx \right)\right) = -\mathcal{I}(x),\quad \forall x > E[X_1]
    \end{aligned}
\end{equation}

% Now, consider $\{X_i\}_{i=1}^{N}$ be the a set of random variables from standard normal distribution. Then by Cramer's theorem, the probability that $\sum X_i$ exceeds $n*a$ for some $a>0$ is approximately given by $P(\frac{\sum X_i}{n}\geq a)=e^{-a^2*n/2}$. 



For more complex distributions, identifying the rate function using logarithmic moment generating function can be challenging. Many methods like contraction principle and exponential tilting exist that extend rate functions from one topological space that satisfies LDP to the topological spaces of interest\cite{den2008large}. For our work, we are interested in the Dawson-G\"artner Projective LDP, that generates the rate function using nested family of projections. 
% \subsection{Ways to generate LDP}
% For more complex distributions, the identifying the rate function using logarithmic moment generating function is not always easy. 
% Let $\{\mu_\epsilon\}_{\epsilon>0}$ satisfy LDP on $\mathcal{X}$ with rate function $\mathcal{I}$.
% \begin{theorem}{Contraction Principle}
% \begin{gather*}
%         \mathcal{T}:\mathcal{X}\to\mathcal{Y}\\
%         \nu=\mu\circ \mathcal{T}^{-1}\\
%         \mathcal{J}(y)=inf_{\{x\in\mathcal{X}\vert \mathcal{T}(x)=y\}}\mathcal{I}(x) \quad \forall y\in\mathcal{Y}
% \end{gather*}
% \end{theorem}
% \begin{theorem}{Exponential Tilting}
% \begin{gather*}
%     \forall F\in \mathrm{C}_b(\mathcal{X}) \\ \nu_\epsilon(dx)=\frac{1}{N_\epsilon}e^{\frac{F(x)}{\epsilon}}\mu_\epsilon(dx)\\
%     \mathcal{J}(x)=\Lambda_F - \left[F(x)-\mathcal{I}(x) \right]\quad x\in\mathcal{X}
% \end{gather*}
% \end{theorem}

\begin{theorem}{Dawson-G\"artner Projective LDP: }
Let $\{\pi^N\}_{N\in\mathbb{N}}$ be a nested family of projections acting on $\mathcal{X}$ s.t. $\cup_{N\in\mathbb{N}}\pi^N$ is the identity. Let $\mathcal{X}^N=\pi^N\mathcal{X}$ and $\mu_\epsilon^N=\mu_0\circ(\pi^N)^{-1}, N\in\mathbb{N}$. If $\forall N\in\mathcal{N}$, the family $\{\mu^N_\epsilon\}_{\epsilon>0}$ satisfies the LDP on $\mathcal{X}^N$ with rate function $\mathcal{I}^N$, then $\{\mu_\epsilon\}_{\epsilon>0}$ satisfies the LDP with rate function $I$ given by,
\[
\begin{aligned}
\mathcal{I}(x)=sup_{N\in\mathbb{N}}\mathcal{I}^N(\pi^N x)\quad x\in\mathcal{X}
\end{aligned}
\]
Since $\mathcal{I}^N(y)=inf_{\{ x\in\mathcal{X}\vert \pi^N(x)=y\}}\mathcal{I}(x),\ y\in\mathcal{Y}$, the supremum defining $\mathcal{I}$ is monotone in N because projections are nested.
\end{theorem}

The theorem allows extending the rate function from a lower projection to higher projection space. The implementation of this theorem in LAD model is discussed in Section \ref{methodology}.


% \begin{theorem}{Sanov's theorem}
% Let $(X_i)_{i\in\mathbb{N}}$ be $\mathbb{R}$-valued r.v. with law $\rho$. Then, law of the empirical distribution $L_n=n^{-1}\sum_{i=1}^n\delta_{X_i} \in \mathcal{M}_1(\mathbb{R})$ given by  $\mu_n$ follows LDP with rate function 
% $\mathcal{I}(\nu)=H(\nu\vert\rho)=\int_\mathbb{R}\nu(dx)log[\frac{d\nu}{d\rho}](x)\quad \forall\nu\in\mathcal{M}_1(\mathbb{R)}$
% \end{theorem}


% {Extending LDP (cont.)}

\subsection{Large Deviations based Anomaly Scoring}
Heterogeneous data with vast diversity pose significant challenges to learning and understanding of the data features. Presence of redundant or irrelevant features act as noise making anomaly detection difficult. However, by dimensionality reduction or feature extraction one might not be able to capture the less significant features of the data. To address this, we use the Dawson-G\"artner Projective theorem in LAD model to compute the rate function for multi-dimensional data. The theorem records the maximum value across all projections which preserves the anomaly score making it optimal to detect anomalies in large and diverse datasets. This anomaly score is used for sampling of the training data for faster convergence of neural networks. See Section\label{methodology}. The model algorithm is presented in Algorithm \ref{alg:lad_score_alg}. 

\begin{algorithm}
\caption{Algorithm 1: LAD Model}
\label{alg:lad_score_alg}
\SetKwProg{generate}{Function \emph{generate}}{}{end}
\textbf{Input}: Dataset $X$ of size $(n,d)$, number of iterations $N_{iter}$, threshold $th$. \\
\textbf{Output}: Anomaly score $\bf{a}$ \\
\textbf{Initialization}: Set initial anomaly score and labels $\bf{a}$ and $\bf{I}$ to zero vectors and, entropy matrix $E=0_{(n,d)}$ where $0_{(n,d)}$ is a zero matrix of size $(n,d)$.\\
\For{each  $s\rightarrow 1\ \KwTo\ N_{iter}$}{
    \begin{enumerate}
        \item Subset $X_{sub}=X[{I}_i==0]$
        \item $X_{normalized}[:,d_i]=\frac{X[:,d_i]-\bar{X_{sub}[:,d_i]}}{cov(X_{sub}[:,d_i])}, \quad \forall d_i\in\{1,\dots,d\}$
        % \item $X_{normalized}=\frac{X-\bar{X_{sub}}}{cov(X_{sub})}$ %\\ Normalized(X_{sub})
        \item $E[i,:]=-X_{normalized}[i]^{2}/2n, \quad \forall i$
        \item $a_i=-max(E[i,:])$
        \item $\bf{a}=\frac{\bf{a}-min(\bf{a})}{max(\bf{a})-min(\bf{a})}$
        % \item Standardize final rate function values and update $\bf{a}_n$
        \item $th=min(th,quantile(\bf{a},0.95)$
        \item $I_i=1$ if $a_i>th,  \quad \forall i$
     \end{enumerate}}
\end{algorithm}




==> LADNN/lit_review_full.tex <==
\section{Related Work}\label{lit_review}
In most settings, real time detection of anomalies is needed to dispatch necessary preventive measures for damage control. Such problem formulation requires collectively monitoring a high dimensional time series database to identify anomalies in real time\footnote{Our work is closely related to anomaly detection on multivariate time series data, high-dimensional anomaly detection and, anomaly detection using large deviations principle. In this section, we limit our review to existing approaches in the related areas.}.

Large deviations theory has been widely applied in the fields of finance \cite{kluppelberg1997large, krasa1992monitoring}, climate modeling \cite{dematteis2018rogue, galfi2019large, ragone2019computation}, statistical mechanics \cite{touchette2009large, derrida2007non}, networks \cite{jakovetic2012distributed, paschalidis2008spatio}, etc. Specially for analysis of time series, the theory of large deviations has proven to be of great interest over recent decades \cite{boettiger2013no, mikosch2016large}. However, these methods are data specific, often study individual time series and are difficult to generalize to other areas of research\cite{oono1989large, chen2018multiscale, yin2015multifractal}. 

Existing anomaly detection algorithms face two major challenges. First challenge is the complexity associated with high dimensional data. A large body of research exists on studying anomalies in high dimensional data \cite{aggarwal2001outlier, angiulli2002fast} but challenges remain. Many anomaly detection algorithms use dimensionality reduction techniques as a pre-processing step to anomaly detection. However, many high dimensional anomalies can only be detected in high dimensional problem settings and dimensionality reduction in such settings can lead to false negatives. 

% Anomaly detection using large deviations principle has 

% Add more reference material here for high dimensional ad

Second challenge is the similarity measure used to study time series data. Detection of anomalous time series have been extensively explored %over time
\cite{gupta2013outlier}. In particular, detecting anomalous time series in a test database with respect to a reference database consisting of normal time series is widely applicable in a number of domains. This problem formulation has been broadly studied over the past few decades\cite{yankov2008disk,chan2005modeling,Chandola:2008, Chandola:2009a}. Most of the techniques are fine tuned to satisfy a particular domain such as studying system health \cite{srivastava2005discovering}, medical data \cite{lin2005approximations}, astronomical data \cite{wei2006saxually, protopapas2006finding} or credit card fraud detection \cite{ferdousi2006unsupervised}. Thus, a more generalized model that can identify anomalous time series in an unsupervised setting within large time series datasets is needed. 



% In particular, anomaly detection in time series data and high dimensional settings have been of exclusive interest \cite{gupta2013outlier,aggarwal2001outlier}. 
% In particular, detection of anomalous series amongst many use similarity measures or Markov models \cite{berndt1994using, Chandola:2008, Chandola:2009a} to identify anomalous time series. These m






==> LADNN/lit_review_old.tex <==
\section{Related Work}\label{lit_review}
In this section, we provide a brief overview of relevant anomaly detection methods which have been proposed for high-dimensional data and for multivariate time-series data. We also discuss other works that have used the large deviations principle for detecting anomalies.

A large body of research exists on studying anomalies in high dimensional data \cite{aggarwal2001outlier, angiulli2002fast} but challenges remain. Many anomaly detection algorithms use dimensionality reduction techniques as a pre-processing step to anomaly detection. However, many high dimensional anomalies can only be detected in high dimensional problem settings and dimensionality reduction in such settings can lead to false negatives. Many methods exist that identify anomalies on high-dimensional data without dimensional reduction or feature selection, e.g. by using distance metrics. {\em Elliptic Envelope} (EE)~\cite{rousseeuw1999fast} fits an ellipse around data centers by fitting a robust covariance estimates.  {\em Isolation Forest} (I-Forest)~\cite{liu2012isolation} uses recursive partitioning by random feature selection and isolating outlier observations. {\em $k$ nearest neighbor outlier detection} (kNN)~\cite{Ramaswamy:2000} uses distance from nearest neighbor to get anomaly scores. {\em local outlier factor} (LOF)~\cite{Breunig:2000} uses deviation in local densities with respect to its neighbors to detect anomalies. {\em k-means\texttt{-{}-}}~\citep{chawla2013k} method uses distance from nearest cluster centers to jointly perform clustering and anomaly detection. {\em Concentration Free Outlier Factor} (CFOF) \cite{angiulli2020cfof} uses a ``reverse nearest neighbor-based score'' which measures the number of nearest neighbors required for a point to have a set proportion of data within its envelope. In particular, methods like I-Forest and CFOF are targeted towards anomaly detection in high dimensional datasets. 

In most settings, real time detection of anomalies is needed to dispatch necessary preventive measures for damage control. Such problem formulation requires collectively monitoring a high dimensional time series database to identify anomalies in real time. Recently, large deviations theory has been widely applied in the fields of climate models \cite{dematteis2018rogue}, statistical mechanics \cite{touchette2009large}, networks \cite{ paschalidis2008spatio}, etc. Specially for analysis of time series, the theory of large deviations has proven to be of great interest over recent decades \cite{boettiger2013no, mikosch2016large}. However, these methods are data specific, often study individual time series and are difficult to generalize to other areas of research.

Anomaly detection for time series have been extensively explored in the literature~\cite{gupta2013outlier}, though most focus has been on identifying anomalous events in a single time-series. While, the task of detecting anomalous time series in a collection of time series has been studied in the past~\cite{yankov2008disk, Chandola:2008, Chandola:2009a}, most of these works have focused on univariate time series and have not shown to scale to long time series data. Our proposed method addresses this issue by using the large deviation principle.

% %
% In most settings, real time detection of anomalies is needed to dispatch necessary preventive measures for damage control. Such problem formulation requires collectively monitoring a high dimensional time series database to identify anomalies in real time\footnote{Our work is closely related to anomaly detection on multivariate time series data, high-dimensional anomaly detection and, anomaly detection using large deviations principle. In this section, we limit our review to existing approaches in the related areas.}.

% Large deviations theory has been widely applied in the fields of climate models \cite{dematteis2018rogue}, statistical mechanics \cite{touchette2009large}, networks \cite{ paschalidis2008spatio}, etc. Specially for analysis of time series, the theory of large deviations has proven to be of great interest over recent decades \cite{boettiger2013no, mikosch2016large}. However, these methods are data specific, often study individual time series and are difficult to generalize to other areas of research.
% \cite{ chen2018multiscale, yin2015multifractal}. 

% Existing anomaly detection algorithms face two major challenges. First challenge is the complexity associated with high dimensional data. A large body of research exists on studying anomalies in high dimensional data \cite{aggarwal2001outlier, angiulli2002fast} but challenges remain. Many anomaly detection algorithms use dimensionality reduction techniques as a pre-processing step to anomaly detection. However, many high dimensional anomalies can only be detected in high dimensional problem settings and dimensionality reduction in such settings can lead to false negatives. 

% Second challenge is the similarity measure used to study time series data. Detection of anomalous time series have been extensively explored %over time
% \cite{gupta2013outlier}. In particular, detecting anomalous time series in a test database with respect to a reference database consisting of normal time series is widely applicable in a number of domains. This problem formulation has been broadly studied over the past\cite{yankov2008disk,Chandola:2008, Chandola:2009a}. Most of the techniques are fine tuned to satisfy a particular domain such as studying system health \cite{srivastava2005discovering}, medical data \cite{lin2005approximations}, astronomical data \cite{protopapas2006finding} or credit card fraud detection \cite{ferdousi2006unsupervised}. Thus, a more generalized model that can identify anomalous time series in an unsupervised setting within large time series datasets is needed. 


% In particular, anomaly detection in time series data and high dimensional settings have been of exclusive interest \cite{gupta2013outlier,aggarwal2001outlier}. 
% In particular, detection of anomalous series amongst many use similarity measures or Markov models \cite{berndt1994using, Chandola:2008, Chandola:2009a} to identify anomalous time series. These m





==> LADNN/related_work.tex <==
\section{Related Work}
Our work closely relates to the area of anomaly detection in time series, large deviations principle based anomaly detection and high dimensional anomaly detection. In this section, we we wish to limit our review to previous approaches in LDP based anomaly detection, anomaly detection in multivariate time series and high dimensional datasets. 


\subsection{Anomaly Detection using Large Deviations Principle}


\subsection{Anomaly Detection in Time Series}

Detection of anomalous time series have been extensively explored over time\cite{gupta2013outlier}. In particular, detecting anomalous time series in a test database with respect to a reference database consisting of normal time series is widely applicable in a number of domains such as studying system health \cite{srivastava2005discovering}, medical data \cite{lin2005approximations}, astronomical data \cite{wei2006saxually,protopapas2006finding} or credit card fraud detection \cite{ferdousi2006unsupervised}. In most settings, real time detection of anomalies is needed to dispatch necessary preventive measures for damage control. This problem formulation has been broadly studied over the past few decades\cite{yankov2008disk,chan2005modeling,Chandola:2008, Chandola:2009a}. 

% Although significant progress has been made in time series anomaly detection, evolving time series is still a challenging component. Anomaly detection in time series can be broadly categorized into two groups: identifying anomalies within each time series that identify sudden anomalous events, and identifying anomalous time series that deviate from non-anomalous trend.



\subsection{Anomaly Detection in High Dimensional Data}
In particular, a large body of research exists on studying anomalies for sequential, time series and temporal datasets \cite{gupta2013outlier,aggarwal2013survey} and high dimensional data \cite{aggarwal2001outlier,angiulli2002fast}. Many anomaly detection algorithms use dimensionality reduction techniques as a pre-processing step to anomaly detection. However, many high dimensional anomalies can be detected in high dimensional problem settings and dimensionality reduction in such settings can lead to false negatives. 


% Historically, anomaly detection algorithm can be broadly classified into score based \cite{} and classification based algorithms \cite{guggilam2019integrated,chawla2013k}. 

==> LADNN/rough.tex <==
Blue Model:
\begin{table}[htb]
  \centering
      \begin{tabular}{|l|c|c|c|c|}
        \hline
        Name & $N$ & $d$ & $c$ \\
        \hline
        MNIST  &  70000  &  256  &  10 \\ 
        kMNIST  &  70000  &  256  &  10 \\
        Fashion MNIST  &  70000  &  256  &  10 \\ 
        Heart-Statlog  &  270  &  13  &  2 \\
      \hline
      \end{tabular}
\end{table}

Orange Model:
\begin{table}[htb]
  \centering
      \begin{tabular}{|l|c|c|c|c|}
        \hline
        Name & $N$ & $d$ & $c$ \\
        \hline
        Concrete  &  1030  &  9  &  2 \\ % O and G
        Abalone  &  4177  &  8  &  2 \\ % R, O, and G
        Sonar  &  208  &  60  &  2 \\ % O and G
        Wine  &  178  &  13  &  3 \\ % R, O and G
        Shuttle  &  58000  &  10  &  2 \\  % O and G
        Skin  &  245057  &  4  &  2 \\
        Glass  &  214  &  9  &  6 \\ % on and off!!
        Balance-Scale  &  625  &  4  &  3 \\ % O and R
        Iris  &  150  &  4  &  3 \\
      \hline
      \end{tabular}
\end{table}

Purple Model:
\begin{table}[htb]
  \centering
      \begin{tabular}{|l|c|c|c|c|}
        \hline
        Name & $N$ & $d$ & $c$ \\
        \hline
        Opt Digits  &  5620  &  63  &  2 \\
        Wave  &  5000  &  22  &  2 \\
        Spambase  &  4601  &  58  &  2 \\
        Pageb  &  5473  &  11  &  2 \\
        Comm And Crime  &  1994  &  102  &  2 \\
        Gas  &  13790  &  129  &  2 \\
        Iono  &  351  &  33  &  2 \\
        Letter Rec  &  20000  &  16  &  26 \\
        % Letter  &  20000  &  16  &  26 \\
        Imgseg  &  2310  &  18  &  7 \\
      \hline
      \end{tabular}
\end{table}

Green Model:
\begin{table}[htb]
  \centering
      \begin{tabular}{|l|c|c|c|c|}
        \hline
        Name & $N$ & $d$ & $c$ \\
        \hline
        Yeast  &  1484  &  8  &  10 \\
        Thy  &  215  &  5  &  3 \\ 
        Tae  &  151  &  3  &  3 \\
        Zoo  &  101  &  16  &  7 \\
        % Wisc  &  699  &  9  &  2 \\ % R and G in smaller pertubations

      \hline
      \end{tabular}
\end{table}


==> LADNN/z_conclusion.tex <==
\section{Conclusion}\label{conclusion}
In this part of the thesis, we propose LAD, a novel scoring algorithm for anomaly detection in large/high-dimensional data. The algorithm successfully handles high dimensions by implementing large deviation theory. Our contributions include reestablishing the advantages of large deviations theory to large and high dimensional datasets. We also present an online extension of the model that is aimed to identify anomalous time series in a multivariate time series data. The model shows vast potential in scalability and performance against baseline methods. The online LAD returns a temporally evolving score for each time series that allows us to study the deviations in trends relative to the complete time series database. 

A potential extension to the model could include anomalous event detection for each individual time series. Another possible future work could be extending the model to enable anomaly detection in multi-modal datasets. Additionally, the online LAD model could be enhanced to use temporally weighted scores prioritizing recent events. 

% inspired score based model to detect anomalies in multivariate time series data setting.  

